Tracking Gaze and Visual Focus of Attention of People Involved in Social Interaction

The visual focus of attention (VFOA) has been recognized as a prominent conversational cue. We are interested in estimating and tracking the VFOAs associated with multi-party social interactions. We note that in this type of situations the participants either look at each other or at an object of interest; therefore their eyes are not always visible. Consequently both gaze and VFOA estimation cannot be based on eye detection and tracking. We propose a method that exploits the correlation between eye gaze and head movements. Both VFOA and gaze are modeled as latent variables in a Bayesian switching state-space model. The proposed formulation leads to a tractable learning procedure and to an efficient algorithm that simultaneously tracks gaze and visual focus. The method is tested and benchmarked using two publicly available datasets that contain typical multi-party human-robot and human-human interactions.

==> tikz_switching_model.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.5cm,inner sep=0pt, minimum size=1cm, thick,main node/.style={circle,draw,font=\sffamily\small\bfseries}]

  \node[main node] (lt) {$\LL_{t-1}$};
  \node[main node] (lt1) [right of=lt, xshift=0.5cm] {$\LL_t$};
  \node[main node, fill=black!30!white] (ht) [below of=lt] {$\H_{t-1}$};
  \node[main node, fill=black!30!white] (ht1) [below of=lt1] {$\H_t$};
  \coordinate[left of=lt] (ltm1);
  \coordinate[right of=lt1] (lt2);
  \node[main node, rectangle] (vt) [above of=lt] {$\V_{t-1}$};
  \node[main node, rectangle] (vt1) [above of=lt1] {$\V_t$};
  \coordinate[left of=vt] (vtm1);
  \coordinate[right of=vt1] (vt2);

  \path[every node/.style={font=\sffamily\small}]
      (lt)  edge node {} (ht)
            edge node {} (lt1)
      (lt1) edge node {} (ht1)
            edge node {} (lt2)
      (ltm1)edge node {} (lt)
      (vt)  edge node {} (lt)
            edge node {} (vt1)
      (vt1) edge node {} (lt1)
            edge node {} (vt2)
      (vtm1)edge node {} (vt)
      ;
\end{tikzpicture}

